Physics implications of recent Dresden-II reactor data

Prompted by the recent Dresden-II reactor data we examine its implications for the determination of the weak mixing angle, paying attention to the effect of the quenching function. We also determine the resulting constraints on the unitarity of the neutrino mixing matrix, as well as on the most general type of nonstandard neutral-current neutrino interactions.

==> Makefile <==
FILENAME=Draft_DRESDEN_PRD_v2
LATEX = pdflatex
BIBTEX = bibtex
PDFTOPS = pdftops
AR = acroread
GV = gv
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"

PSFILE = Draft_DRESDEN_PRD_v2.ps 
PDFFILE = Draft_DRESDEN_PRD_v2.pdf

COPY = if test -r Draft_DRESDEN_PRD_v2.toc; then cp Draft_DRESDEN_PRD_v2.toc Draft_DRESDEN_PRD_v2.toc.bak; fi 
RM = /bin/rm -f

CLEAN=rm -f Draft_DRESDEN_PRD_v2.aux Draft_DRESDEN_PRD_v2.log Draft_DRESDEN_PRD_v2.dvi Draft_DRESDEN_PRD_v2.toc Draft_DRESDEN_PRD_v2.out Draft_DRESDEN_PRD_v2.blg Draft_DRESDEN_PRD_v2.mtc Draft_DRESDEN_PRD_v2.mtc1 Draft_DRESDEN_PRD_v2.rel Draft_DRESDEN_PRD_v2.vrb Draft_DRESDEN_PRD_v2.end Draft_DRESDEN_PRD_v2.spl *.aux *~ \#*

WARNING=egrep -i "(Reference|Citation).*undefined" Draft_DRESDEN_PRD_v2.log ; true

HELP=cat /home/jv/bin/help/MakePDFLatexMakefile.help

main:	Draft_DRESDEN_PRD_v2.tex pdf

pdf:	$(PDFFILE)
	$(WARNING)  

all:	$(PDFFILE) $(PSFILE)
	$(WARNING)  

ps:	$(PSFILE) 
	$(WARNING)

gv:	$(PSFILE)
	$(GV) $(PSFILE) &
	$(WARNING)

	$(WARNING)

ar:	$(PDFFILE)
	$(AR) $(PDFFILE) &

%.pdf:	%.tex
	python3.6 /usr/local/bin/PhysBiblio.exe tex bibliography.bib './Draft_DRESDEN_PRD_v2.tex' 
	$(COPY);$(LATEX) $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ;true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	if [  'cmp -s $*.toc $*.toc.bak'  ]; then $(LATEX) $< ; fi
	$(RM) $*.toc.bak

%.ps:	%.pdf
	$(PDFTOPS) $<

clean:	
	$(CLEAN)

realclean: 	
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).pdf $(FILENAME).bbl

help:
	$(HELP)

complete: realclean pdf clean


